Robust Machine Learning for Encrypted Traffic Classification

Desktops and laptops can be maliciously exploited to violate privacy. In this paper, we consider the daily battle between the passive attacker who is targeting a specific user against a user that may be adversarial opponent. In this scenario, while the attacker tries to choose the best vector attack by surreptitiously monitoring the victims encrypted network traffic in order to identify users parameters such as the Operating System (OS), browser and apps. The user may use tools such as a Virtual Private Network (VPN) or even change protocols parameters to protect his/her privacy. We provide a large dataset of more than 20,000 examples for this task. We run a comprehensive set of experiments, that achieves high (above 85) classification accuracy, robustness and resilience to changes of features as a function of different network conditions at test time. We also show the effect of a small training set on the accuracy.

==> RandomForest_results.tex <==
Training_Data_Set_Size,Combined_Features,Common,New,Combined_no_peaks,Combined_no_SSL,Combined_no_TCP,Peaks,Stats,Common_stats
50,67.12,61.07,66.09,67.27,64.78,65.26,56.19,61.27,61.01
100,74.45,69.12,73.88,75.31,70.67,73.36,61.99,69.21,68.91
200,81.81,75.13,80.62,81.24,78.25,80.25,67.75,76.17,73.86
300,84.87,79.08,83.53,84.84,82.37,84.04,71.51,80.44,78.51
400,86.36,81.85,85.37,86.32,84.26,86.10,74.08,82.82,81.13
500,87.81,83.61,86.81,88.14,85.83,87.26,75.90,84.34,82.80
600,89.46,85.29,87.82,89.10,87.46,88.67,77.50,85.85,84.63
700,89.90,86.20,88.49,89.75,87.95,89.55,78.17,86.95,85.46
800,90.88,86.94,89.23,90.57,88.85,90.46,78.88,87.95,86.77
900,91.60,87.85,90.22,91.48,89.66,91.26,79.66,88.54,87.45
1000,91.85,88.64,90.76,91.88,90.01,91.39,80.37,89.20,88.10
2000,94.55,92.12,93.41,94.46,93.14,94.21,83.99,92.41,91.69
5000,96.61,94.62,95.32,96.44,95.52,96.56,87.99,95.03,94.49
10000,97.53,96.10,96.65,97.35,96.79,97.46,90.42,96.49,96.03
14443,97.91,96.68,97.00,97.75,97.16,97.81,91.83,97.03,96.59


==> RandomForest_times_test_CHECK.tex <==
Training_Data_Set_Size,Stats,Combined_no_TCP,Peaks,Common,Common_stats,Combined_no_peaks,Combined_Features,New,Combined_no_SSL
50,0.000050,0.000040,0.000024,0.000027,0.000032,0.000032,0.000044,0.000026,0.000042
100,0.000047,0.000048,0.000039,0.000058,0.000029,0.000032,0.000040,0.000042,0.000047
200,0.000040,0.000039,0.000052,0.000032,0.000047,0.000057,0.000047,0.000039,0.000044
300,0.000040,0.000048,0.000042,0.000044,0.000048,0.000040,0.000047,0.000047,0.000058
400,0.000053,0.000057,0.000052,0.000055,0.000048,0.000047,0.000052,0.000047,0.000053
500,0.000061,0.000065,0.000057,0.000055,0.000047,0.000057,0.000040,0.000065,0.000060
600,0.000055,0.000048,0.000052,0.000057,0.000055,0.000040,0.000052,0.000042,0.000053
700,0.000050,0.000048,0.000052,0.000052,0.000055,0.000060,0.000057,0.000048,0.000052
800,0.000052,0.000044,0.000044,0.000066,0.000053,0.000053,0.000057,0.000048,0.000040
900,0.000069,0.000068,0.000060,0.000068,0.000060,0.000057,0.000057,0.000053,0.000060
1000,0.000060,0.000057,0.000052,0.000057,0.000057,0.000048,0.000052,0.000068,0.000052
2000,0.000066,0.000060,0.000052,0.000055,0.000055,0.000058,0.000066,0.000052,0.000065
5000,0.000066,0.000060,0.000047,0.000061,0.000060,0.000057,0.000058,0.000066,0.000065
10000,0.000068,0.000068,0.000068,0.000071,0.000068,0.000057,0.000065,0.000069,0.000055
14443,0.000060,0.000061,0.000074,0.000060,0.000055,0.000057,0.000060,0.000057,0.000073


==> RandomForest_times_train_CHECK.tex <==
Training_Data_Set_Size,Stats,Combined_no_TCP,Peaks,Common,Common_stats,Combined_no_peaks,Combined_Features,New,Combined_no_SSL
50.00,2.61,2.44,2.31,2.32,2.43,2.37,2.4,2.26,2.63
100.00,2.77,2.89,2.77,2.93,2.58,2.61,2.63,2.69,2.86
200.00,2.81,2.82,2.84,2.7,2.82,2.92,2.91,2.72,2.85
300.00,2.97,3.12,2.94,2.98,3.09,2.89,3.14,3.08,3.32
400.00,3.33,3.2,3.09,3.17,2.99,3.15,3.13,3.1,3.15
500.00,3.52,3.57,3.52,3.23,3.39,3.42,3.18,3.47,3.44
600.00,3.56,3.46,3.37,3.55,3.44,3.24,3.36,3.16,3.41
700.00,3.53,3.55,3.57,3.5,3.56,3.52,3.54,3.38,3.55
800.00,3.65,3.53,3.61,3.73,3.64,3.54,3.67,3.57,3.59
900.00,4,4,3.79,3.96,3.72,3.7,3.69,3.58,3.8
1000.00,4.06,4.03,3.96,3.84,3.98,3.89,3.9,3.98,4.02
2000.00,4.56,4.42,4.17,4.31,4.23,4.25,4.35,4.04,4.45
5000.00,5.79,5.58,4.9,5.46,5.22,5.38,5.4,4.97,5.72
10000.00,8.36,8.45,7.96,7.85,7.61,7.23,7.68,7.21,7.93
14443.00,10.57,10.23,10.04,9.14,9.49,8.85,9.92,8.1,10.55


==> Tuple_results.tex <==
ML,Combined_Features,Common,New,Combined_no_peaks,Combined_no_SSL,Combined_no_TCP,Peaks,Stats,Common_stats,,
0,96.7,94.45,95.73,96.44,95.91,96.64,86.94,95.42,94.39,KNN,
1,96,94,92.1,95.91,94.43,95.77,83.15,94.02,93.8,SVM+RBF,
2,97.91,96.68,97,97.75,97.16,97.81,91.83,97.03,96.59,RF,
3,97.97,96.42,96.89,97.77,97.21,97.87,90.78,96.94,96.37,SVM+MAP,
4,97.86,95.15,96.52,97.47,96.78,97.59,86.36,96.2,94.65,SVM+SIM,threshold


==> chrome_costarica4k_720_auto.tex <==
0,270
1,0
2,0
3,8256
4,524086
5,1695475
6,2845537
7,2528992
8,846981
9,610940
10,1525430
11,0
12,436625
13,1821256
14,0
15,0
16,309412
17,1563782
18,388294
19,54
20,0
21,0
22,2213821
23,648
24,0
25,398073
26,0
27,0
28,1632533
29,0
30,0
31,2119289
32,291797
33,0
34,0
35,2160699
36,0
37,0
38,1440462
39,945213
40,0
41,0
42,1575529
43,0
44,0
45,2206042
46,0
47,0
48,0
49,543814
50,972587
51,1163367
52,0
53,0
54,0
55,0
56,0
57,0
58,0
59,0
60,0
61,0
62,0
63,0
64,0
65,0
66,2012707
67,54
68,0
69,108
70,0
71,0
72,0
73,108
74,0
75,0
76,0
77,683877
78,1111076
79,0
80,0
81,0
82,0
83,0
84,0
85,0
86,4464
87,575125
88,1867724
89,0
90,0
91,0
92,0
93,0
94,0
95,0
96,0
97,0
98,0
99,1803957
100,0
101,0
102,0
103,0
104,0
105,0
106,0
107,0
108,508542
109,0
110,0
111,0
112,0
113,0
114,1451680
115,0
116,0
117,0
118,0
119,0
120,0
121,0
122,0
123,0
124,0
125,2207992
126,0
127,0
128,0
129,0
130,0
131,0
132,0
133,0
134,0
135,1430561
136,403345
137,0
138,0
139,0
140,0
141,0
142,0
143,0
144,0
145,526724
146,1085315
147,1113975
148,0
149,0
150,0
151,0
152,0
153,0
154,0
155,0
156,0
157,0
158,0
159,0
160,0
161,0
162,0
163,2151156
164,0
165,0
166,0
167,0
168,0
169,0
170,0
171,0
172,194038
173,2389574
174,0
175,0
176,0
177,0
178,0
179,0
180,0
181,0
182,0
183,907441
184,1297737
185,0
186,0
187,0
188,0
189,0
190,0
191,0
192,0
193,162
194,145453
195,774114
196,0
197,0
198,0
199,0
200,0
201,0
202,0
203,0
204,0
205,0
206,0
207,0
208,0
209,0
210,0
211,0
212,0
213,0
214,0
215,0
216,0
217,0
218,0
219,0
220,0
221,0
222,0
223,0
224,0
225,108


==> cipher_browser_new.tex <==
ML,Combined_Features,Common,New,Combined_no_peaks,Combined_no_SSL,Combined_no_TCP,Peaks,Stats,Common_stats,,
0,93.64,89.92,87.94,92.57,89.54,93.58,91.73,91.08,90.53,KNN,
1,82.50,89.45,81.09,82.07,89.08,85.84,85.33,88.99,90.01,SVM+RBF,
2,96.25,89.97,91.42,93.31,90.99,96.01,92.46,90.72,89.95,RF,
3,90.15,91.41,93.76,89.10,91.28,88.63,85.40,91.37,85.48,SVM+MAP,dist
4,83.81,85.44,81.31,91.44,86.17,84.99,85.26,85.91,85.48,SVM+SIM,threshold


==> cipher_os_browser_new.tex <==
ML,Combined_Features,Common,New,Combined_no_peaks,Combined_no_SSL,Combined_no_TCP,Peaks,Stats,Common_stats,,
0,91.89,89.85,88.92,91.57,90.81,89.01,73.82,89.21,88.50,KNN,
1,80.11,90.43,80.42,80.96,90.24,79.51,68.00,87.96,89.17,SVM+RBF,
2,96.66,91.17,95.99,96.12,91.53,96.23,74.31,91.21,91.06,RF,
3,93.11,91.10,94.76,92.78,92.15,92.20,72.18,92.55,89.95,SVM+MAP,dist
4,91.79,88.61,75.78,91.19,91.66,89.95,68.05,91.01,88.34,SVM+SIM,threshold


==> knn_results.tex <==
Training_Data_Set_Size,Combined_Features,Common,New,Combined_no_peaks,Combined_no_SSL,Combined_no_TCP,Peaks,Stats,Common_stats
50,64.63,59.32,67.56,67.07,63.75,61.70,53.41,59.70,58.94
100,73.32,69.37,70.85,74.90,68.16,71.33,59.57,68.65,68.74
200,77.81,73.69,76.83,78.32,75.95,75.58,65.29,72.98,73.36
300,82.47,77.51,80.19,83.11,80.25,81.37,68.83,77.52,77.48
400,84.59,79.16,83.28,84.43,81.74,83.51,70.38,79.93,78.75
500,85.57,80.09,84.24,85.59,82.53,84.50,72.28,81.48,80.13
600,86.45,82.32,85.74,86.70,84.51,85.80,73.61,82.75,81.99
700,87.36,83.19,86.02,86.98,84.48,86.62,74.17,83.77,82.77
800,88.42,83.85,86.80,88.10,86.43,87.74,74.68,84.66,83.52
900,89.22,84.98,87.54,89.06,86.92,88.53,75.42,85.52,84.53
1000,89.49,85.11,88.11,89.46,87.17,88.70,75.91,86.07,85.00
2000,92.11,88.89,91.12,91.87,90.89,91.64,79.74,89.91,88.58
5000,94.79,91.83,93.88,94.63,93.75,94.68,83.74,93.03,91.72
10000,96.30,93.75,95.31,95.92,95.29,96.15,85.85,94.79,93.64
14443,96.70,94.45,95.73,96.44,95.91,96.64,86.94,95.42,94.39


==> knn_times_test_CHECK.tex <==
Training_Data_Set_Size,Stats,Combined_no_TCP,Peaks,Common,Common_stats,Combined_no_peaks,Combined_Features,New,Combined_no_SSL
50,0.000008,0.000008,0.000008,0.000008,0.000008,0.000006,0.000008,0.000008,0.000010
100,0.000010,0.000013,0.000008,0.000013,0.000011,0.000010,0.000011,0.000010,0.000008
200,0.000013,0.000015,0.000011,0.000013,0.000013,0.000013,0.000015,0.000015,0.000015
300,0.000018,0.000023,0.000013,0.000018,0.000016,0.000018,0.000016,0.000013,0.000018
400,0.000021,0.000023,0.000018,0.000019,0.000018,0.000019,0.000021,0.000019,0.000021
500,0.000029,0.000026,0.000021,0.000024,0.000021,0.000023,0.000021,0.000026,0.000031
600,0.000034,0.000026,0.000024,0.000031,0.000029,0.000027,0.000032,0.000026,0.000034
700,0.000039,0.000037,0.000027,0.000032,0.000032,0.000031,0.000037,0.000031,0.000037
800,0.000040,0.000040,0.000031,0.000036,0.000039,0.000037,0.000039,0.000032,0.000042
900,0.000044,0.000039,0.000037,0.000040,0.000040,0.000042,0.000042,0.000039,0.000045
1000,0.000045,0.000044,0.000036,0.000042,0.000042,0.000040,0.000044,0.000037,0.000047
2000,0.000081,0.000073,0.000055,0.000060,0.000068,0.000061,0.000076,0.000061,0.000086
5000,0.000129,0.000145,0.000097,0.000118,0.000111,0.000120,0.000132,0.000103,0.000141
10000,0.000236,0.000233,0.000141,0.000194,0.000191,0.000147,0.000233,0.000118,0.000213
14443,0.000288,0.000283,0.000165,0.000247,0.000241,0.000257,0.000284,0.000183,0.000312


==> knn_times_test_CHECK_old.tex <==
Training_Data_Set_Size	Stats	Combined_no_TCP	Peaks	Common	Common_stats	Combined_no_peaks	Combined_Features	New	Combined_no_SSL
50	0.000008	0.000008	0.000008	0.000008	0.000008	0.000006	0.000008	0.000008	0.000010
100	0.000010	0.000013	0.000008	0.000013	0.000011	0.000010	0.000011	0.000010	0.000008
200	0.000013	0.000015	0.000011	0.000013	0.000013	0.000013	0.000015	0.000015	0.000015
300	0.000018	0.000023	0.000013	0.000018	0.000016	0.000018	0.000016	0.000013	0.000018
400	0.000021	0.000023	0.000018	0.000019	0.000018	0.000019	0.000021	0.000019	0.000021
500	0.000029	0.000026	0.000021	0.000024	0.000021	0.000023	0.000021	0.000026	0.000031
600	0.000034	0.000026	0.000024	0.000031	0.000029	0.000027	0.000032	0.000026	0.000034
700	0.000039	0.000037	0.000027	0.000032	0.000032	0.000031	0.000037	0.000031	0.000037
800	0.000040	0.000040	0.000031	0.000036	0.000039	0.000037	0.000039	0.000032	0.000042
900	0.000044	0.000039	0.000037	0.000040	0.000040	0.000042	0.000042	0.000039	0.000045
1000	0.000045	0.000044	0.000036	0.000042	0.000042	0.000040	0.000044	0.000037	0.000047
2000	0.000081	0.000073	0.000055	0.000060	0.000068	0.000061	0.000076	0.000061	0.000086
5000	0.000129	0.000145	0.000097	0.000118	0.000111	0.000120	0.000132	0.000103	0.000141
10000	0.000236	0.000233	0.000141	0.000194	0.000191	0.000147	0.000233	0.000118	0.000213
14443	0.000288	0.000283	0.000165	0.000247	0.000241	0.000257	0.000284	0.000183	0.000312


==> knn_times_train_CHECK.tex <==
Training_Data_Set_Size,Stats,Combined_no_TCP,Peaks,Common,Common_stats,Combined_no_peaks,Combined_Features,New,Combined_no_SSL
50,2.23,2.22,2.25,2.21,2.22,2.24,2.16,2.2,2.2
100,2.5,2.54,2.53,2.45,2.46,2.5,2.49,2.46,2.51
200,2.61,2.62,2.51,2.58,2.57,2.63,2.6,2.56,2.61
300,2.73,2.77,2.65,2.69,2.82,2.74,2.64,2.73,2.7
400,2.99,2.9,2.86,2.89,2.89,2.93,2.9,2.92,2.96
500,3.15,3.16,2.97,3.06,3,3.07,3.1,3.02,3.13
600,3.15,3.31,3.01,3.14,3.1,3.22,3.3,3.14,3.34
700,3.41,3.48,3.12,3.28,3.23,3.31,3.42,3.19,3.44
800,3.8,3.81,3.36,3.56,3.5,3.74,3.86,3.46,3.88
900,3.91,4.09,3.4,3.73,3.66,3.86,4.07,3.65,4
1000,4.23,4.42,3.61,3.98,3.97,4.15,4.39,3.88,4.37
2000,7.49,7.81,5.55,6.59,6.65,7.25,7.43,6.19,7.73
5000,23.04,25.58,13.41,18.58,18.09,20.97,27.23,15.77,24.6
10000,95.77,113.4,30.97,60.65,60.67,111.9,121.32,50.22,119.96
14443,211.23,254.23,53.32,130.48,120.68,194.23,283.3,89.49,236.78


==> real_time_results_10min.tex <==
ML,Combined_Features,Common,New,Combined_no_peaks,Combined_no_SSL,Combined_no_TCP,Peaks,Stats,Common_stats,,
0,93.87,91.42,91.22,93.40,92.75,93.71,81.96,92.40,91.32,KNN,
1,92.25,90.95,89.13,92.70,91.56,92.65,78.33,91.01,90.78,SVM+RBF,
2,95.51,93.87,93.23,95.25,94.58,95.31,87.45,94.38,93.84,RF,
3,95.30,93.32,92.91,95.03,94.41,95.32,86.00,94.17,93.25,SVM+MAP,dist
4,95.09,91.87,92.23,94.79,93.56,94.87,81.89,92.69,91.54,SVM+SIM,threshold


==> real_time_results_10sec.tex <==
ML,Combined_Features,Common,New,Combined_no_peaks,Combined_no_SSL,Combined_no_TCP,Peaks,Stats,Common_stats,,
0,92.02774668,87.78568265,89.46154463,92.03476422,88.62015526,91.74026111,77.15616887,87.86289524,87.70855363,KNN,
1,91.38963489,87.05646083,86.10297765,91.04612698,87.93290594,91.15824292,71.02096954,87.14059264,87.02140509,SVM+RBF,
2,94.02606887,91.41773454,91.2074763,94.08917018,91.99973552,93.89988836,83.08801444,91.71225486,91.34062027,RF,
3,94.07514493,90.93395943,91.38274025,93.87181083,91.69118995,93.99800854,82.82854002,91.1022378,90.84982025,SVM+MAP,dist
4,93.75959903,88.92864429,89.83312514,93.52825131,90.68857417,93.47913591,79.8907132,89.55267185,88.42376987,SVM+SIM,threshold


==> real_time_results_1min.tex <==
ML,Combined_Features,Common,New,Combined_no_peaks,Combined_no_SSL,Combined_no_TCP,Peaks,Stats,Common_stats,,
0,92.20810457,88.96590554,90.00261453,92.06283775,90.1544842,92.05622837,79.9260168,89.62623089,88.84044723,KNN,
1,91.60719169,88.37820051,87.3018832,91.3430694,89.32905297,91.35627289,75.4886668,88.84700646,88.35178916,SVM+RBF,
2,94.45982757,92.22789564,91.87134233,94.30134416,93.03351181,94.20890877,84.89828182,92.61092138,92.10906416,RF,
3,94.25512211,91.210969,91.95716615,93.85891468,92.37977185,94.13626664,84.05306389,91.83830632,91.09871637,SVM+MAP,dist
4,93.72683827,89.54693794,91.41570717,93.27784085,91.34965697,93.58158017,79.62888031,90.38559883,89.31582331,SVM+SIM,threshold


==> real_time_results_1sec.tex <==
ML,Combined_Features,Common,New,Combined_no_peaks,Combined_no_SSL,Combined_no_TCP,Peaks,Stats,Common_stats,,
0,91.67,87.28,87.10,91.55,88.89,91.58,71.91,88.40,87.18,KNN,
1,91.31,87.36,86.12,91.51,88.32,90.94,71.13,87.39,87.44,SVM+RBF,
2,93.85,90.71,90.13,93.76,91.54,93.66,77.98,91.31,90.70,RF,
3,94.32,90.49,89.76,93.86,91.65,94.20,77.27,91.22,90.41,SVM+MAP,dist
4,93.68,89.00,88.98,93.28,90.54,93.64,76.53,90.21,88.41,SVM+SIM,threshold


==> results_app_clean.tex <==
ML,Combined_Features,Common,New,Combined_no_peaks,Combined_no_SSL,Combined_no_TCP,Peaks,Stats,Common_stats
0,97.66,96.79,96.61,97.35,97.45,97.59,93.92,97.28,96.73
1,96.35,95.94,93.6,96.53,95.94,96.26,90.11,95.93,95.7
2,98.22,97.8,97.51,98.09,98.1,98.18,95.4,98.03,97.76
3,98.28,97.82,97.44,98.16,98.14,98.20,95.29,97.99,97.74
4,95.46,94.61,96.06,95.50,95.11,95.17,92.72,94.65,94.39


==> results_browser_clean.tex <==
ML,Combined_Features,Common,New,Combined_no_peaks,Combined_no_SSL,Combined_no_TCP,Peaks,Stats,Common_stats,,
0,98.9,96.36,98.73,98.95,97.55,98.87,93.77,97.14,96.34,KNN,
1,98.7,96.22,98.08,98.62,96.72,98.33,89.97,96.39,95.8,SVM+RBF,
2,99.29,97.98,99.09,99.24,98.46,99.29,95.59,98.21,97.94,RF,
3,99.44,97.93,99.10,99.46,98.52,99.40,95.31,98.27,97.91,SVM+MAP,dist
4,99.03,93.87,98.58,98.94,95.07,98.93,91.78,94.20,93.77,SVM+SIM,threshold


==> results_os_clean.tex <==
ML,Combined_Features,Common,New,Combined_no_peaks,Combined_no_SSL,Combined_no_TCP,Peaks,Stats,Common_stats,,
0,99.95,99.74,99.95,99.96,99.98,99.75,91.52,99.58,99.61,KNN,
1,100,99.58,100,100,100,99.61,87.4,99.26,99.32,SVM+RBF,
2,100,99.93,100,100,100,99.86,95.1,99.79,99.8,RF,
3,100.00,99.91,99.99,99.99,100.00,99.87,94.19,99.81,99.82,SVM+MAP,dist
4,100.00,99.65,100.00,99.99,100.00,99.76,89.64,99.39,99.46,SVM+SIM,threshold


==> svmrbf_results.tex <==
Training_Data_Set_Size,Combined_Features,Common,New,Combined_no_peaks,Combined_no_SSL,Combined_no_TCP,Peaks,Stats,Common_stats
50,64.37,58.42,61.32,67.49,59.02,63.31,47.97,57.54,57.77
100,72.20,66.22,71.46,72.33,66.94,69.33,54.61,65.20,65.86
200,76.44,70.72,76.78,77.53,72.23,74.88,60.58,70.05,70.82
300,80.51,74.33,79.92,80.18,76.61,79.91,63.92,73.88,73.91
400,81.73,75.88,81.11,82.29,77.55,81.44,65.51,74.90,75.77
500,83.85,78.46,82.76,84.11,79.17,83.47,66.22,78.19,78.30
600,85.25,79.57,83.63,84.80,81.03,84.58,67.93,79.59,79.55
700,85.19,80.01,83.89,85.07,81.62,85.24,68.21,80.23,79.93
800,86.55,82.19,84.60,86.20,83.00,85.95,68.93,81.39,81.98
900,86.95,83.06,85.36,87.17,83.61,86.61,69.10,82.05,82.79
1000,87.82,83.60,85.89,87.92,84.03,87.07,70.16,82.99,83.69
2000,90.73,86.93,88.65,91.15,88.26,90.83,74.68,87.16,86.86
5000,93.98,90.78,91.71,93.79,91.95,93.62,79.03,91.13,90.80
10000,95.35,93.06,92.94,95.36,93.73,95.35,82.13,93.13,92.94
14443,95.89,94.00,93.56,95.91,94.43,95.77,83.15,94.02,93.99


==> svmrbf_times_test_CHECK.tex <==
Training_Data_Set_Size,Stats,Combined_no_TCP,Peaks,Common,Common_stats,Combined_no_peaks,Combined_Features,New,Combined_no_SSL
50,0.000011,0.000013,0.000008,0.000010,0.000010,0.000011,0.000015,0.000010,0.000013
100,0.000021,0.000024,0.000015,0.000019,0.000018,0.000021,0.000026,0.000018,0.000023
200,0.000037,0.000042,0.000027,0.000032,0.000032,0.000036,0.000042,0.000031,0.000039
300,0.000050,0.000057,0.000039,0.000044,0.000044,0.000052,0.000057,0.000044,0.000053
400,0.000068,0.000073,0.000048,0.000058,0.000057,0.000065,0.000074,0.000053,0.000073
500,0.000078,0.000082,0.000053,0.000061,0.000063,0.000068,0.000086,0.000055,0.000073
600,0.000089,0.000092,0.000068,0.000073,0.000074,0.000082,0.000092,0.000068,0.000087
700,0.000099,0.000100,0.000076,0.000081,0.000073,0.000089,0.000097,0.000076,0.000097
800,0.000105,0.000108,0.000074,0.000090,0.000090,0.000086,0.000110,0.000078,0.000107
900,0.000111,0.000107,0.000087,0.000097,0.000086,0.000089,0.000121,0.000087,0.000103
1000,0.000113,0.000121,0.000092,0.000094,0.000100,0.000110,0.000113,0.000084,0.000113
2000,0.000163,0.000124,0.000129,0.000137,0.000136,0.000142,0.000168,0.000128,0.000144
5000,0.000202,0.000191,0.000160,0.000178,0.000170,0.000170,0.000218,0.000149,0.000208
10000,0.000255,0.000246,0.000278,0.000234,0.000216,0.000242,0.000312,0.000202,0.000273
14443,0.000321,0.000283,0.000363,0.000263,0.000265,0.000237,0.000294,0.000221,0.000313


==> svmrbf_times_train_CHECK.tex <==
Training_Data_Set_Size,Stats,Combined_no_TCP,Peaks,Common,Common_stats,Combined_no_peaks,Combined_Features,New,Combined_no_SSL
50,1.31,1.32,1.30,1.29,1.34,1.29,1.32,1.32,1.34
100,1.70,1.69,1.67,1.63,1.65,1.69,1.78,1.62,1.70
200,2.15,2.20,1.92,2.04,2.10,2.28,2.33,1.90,2.20
300,2.61,2.64,2.39,2.56,2.52,2.67,2.65,2.46,2.62
400,2.69,2.72,2.65,2.68,2.58,2.74,2.76,2.73,2.67
500,2.94,2.95,2.70,2.73,2.78,2.91,2.94,2.76,2.88
600,3.11,3.13,2.76,2.81,2.85,2.99,3.18,2.80,3.12
700,3.39,3.48,2.79,3.09,3.02,3.26,3.60,2.78,3.39
800,3.93,4.10,3.13,3.50,3.52,3.81,4.18,3.12,3.99
900,4.39,4.48,3.49,3.87,3.81,4.12,4.61,3.33,4.43
1000,4.94,5.07,3.73,4.20,4.31,4.53,5.15,3.62,4.88
2000,10.89,11.36,7.59,8.85,8.77,9.74,11.89,6.85,11.12
5000,41.87,44.10,32.17,32.77,32.30,35.61,46.82,23.72,42.89
10000,156.21,177.88,110.94,125.42,110.61,141.84,225.47,81.91,169.12
14443,372.33,376.07,235.92,237.96,228.85,278.19,429.59,152.24,359.17


==> vpn_os_browser.tex <==
ML,Combined_Features,Common,New,Combined_no_peaks,Combined_no_SSL,Combined_no_TCP,Peaks,Stats,Common_stats,Combined_FeaturesEB,CommonEB,NewEB,Combined_no_peaksEB,Combined_no_SSLEB,Combined_no_TCPEB,PeaksEB,StatsEB,Common_statsEB
0,58.33,41.67,20,53.33,28.33,31.67,6.67,15,43.33,0.097182532,0.084983659,0.290593263,0.062360956,0.1,0.143372088,0.081649658,0.084983659,0.084983659
1,63.33,21.67,56.67,60,50,60,1.67,26.67,21.67,0.081649658,0.091287093,0.281858909,0.084983659,0.033333333,0.062360956,0,0.040824829,0.124721913
2,65,50,26.67,70,48.33,60,6.67,46.67,48.33,0.113038833,0.074535599,0.163299316,0.062360956,0.161589329,0.062360956,0.066666667,0.084983659,0.139443338
3,83.33,50,53.33,80,70,65,6.67,48.33,40,0,0,0,0,0,0,0,0,0
4,75,56.67,38.33,81.67,68.33,63.33,15,33.33,50,0,0,0,0,0,0,0,0,0

